Reactive User Behavior and Mobility Models

In this paper, we present a set of simulation models to more realistically mimic the behaviour of users reading messages. We propose a User Behaviour Model, where a simulated user reacts to a message by a flexible set of possible reactions (e.g. ignore, read, like, save, etc.) and a mobility-based reaction (visit a place, run away from danger, etc.). We describe our models and their implementation in OMNeT++. We strongly believe that these models will significantly contribute to the state of the art of simulating realistically opportunistic networks.

==> eval.tex <==
% !TEX root = report.tex

\section{Evaluation Results}\label{sec:eval}

We have implemented our models in the OMNeT++ network simulator. The complete model stack is presented in Figure~\ref{fig:omnet-stack} and consists of:

\begin{itemize}
\item User: 
\item ReactiveSWIM:
\item EventApplication:
\item Gossiping:
\item Link layer:
\end{itemize}





==> related.tex <==
% !TEX root = report.tex

\section{Motivation and Related Works}\label{sec:related}


